Characterizing the Networks Sending Enterprise Phishing Emails

Phishing attacks on enterprise employees present one of the most costly and potent threats to organizations. We explore an understudied facet of enterprise phishing attacks: the email relay infrastructure behind successfully delivered phishing emails. We draw on a dataset spanning one year across thousands of enterprises, billions of emails, and over 800,000 delivered phishing attacks. Our work sheds light on the network origins of phishing emails received by real-world enterprises, differences in email traffic we observe from networks sending phishing emails, and how these characteristics change over time. Surprisingly, we find that over one-third of the phishing email in our dataset originates from highly reputable networks, including Amazon and Microsoft. Their total volume of phishing email is consistently high across multiple months in our dataset, even though the overwhelming majority of email sent by these networks is benign. In contrast, we observe that a large portion of phishing emails originate from networks where the vast majority of emails they send are phishing, but their email traffic is not consistent over time. Taken together, our results explain why no singular defense strategy, such as static blocklists (which are commonly used in email security filters deployed by organizations in our dataset), is effective at blocking enterprise phishing. Based on our offline analysis, we partnered with a large email security company to deploy a classifier that uses dynamically updated network-based features. In a production environment over a period of 4.5 months, our new detector was able to identify 3-5% more enterprise email attacks that were previously undetected by the company's existing classifiers.

==> acknowledgements.tex <==
\section*{Acknowledgements}
This work was supported in part by the NSF CNS-2106530 and CNS-2143868 awards, and the UCSD CSE Postdoctoral Fellows program.

\clearpage

==> case_studies-old.tex <==
\section{Case Studies}
\label{sec:caseStudies}
\enew{Now, we investigate several nuances in network behavior that the aggregate analysis in the previous section does not fully capture by examining some illustrative examples of ASes (and the IP addresses contained within them) in both the low and high-risk category. First, we take a deeper dive into the two prominent low-risk networks (Amazon and Microsoft) ~(\S\ref{sec:case:low_risk}). Then, we explore two contrasting examples of high-risk networks: one that remains high risk across the three months~(\S\ref{sec:case-study-persistent}), and one that is comparatively transient, sending phishing emails in short bursts in a single month ~(\S\ref{sec:case-study-bursty}).} % Perhaps summarize the takeaways of this section here before the reader gets bogged down in the details? I'll see if its too repetitive though.


% tie the sections together a bit more by offering some motivations/context to the case studies.
% \enew{In the previous section, we found several nuances in the network infrastructure used to send phishing email. In this section, we investigate in more detail and offer explanations for their behavior by discussing specific networks and IP addresses in both the low and high-risk category. First, we examine two prominent low-risk networks, namely the public cloud networks of Amazon and Microsoft~(\S\ref{sec:case:low_risk}). We also explore two examples of high-risk networks: one that sends phishing emails in two bursts in a single month~(\S\ref{sec:case-study-bursty}) and one that remains high risk across the three months~(\S\ref{sec:case-study-persistent}).}

% Perhaps also summarize the takeaways of this section here before the reader gets bogged down in the details.
% \enew{Within our case studies, we found that attack campaigns originating from both high-risk and low-risk networks are often short-lived, which is in line with prior work on phishing campaigns \cite{simoiu2020targeted}. However, some attackers also use Internet hosting providers (and the same IP addresses) over long periods of time.}
% \enew{Low-risk Network Attack vectors: email account takeover, dedicated phishing server (sending spoofed emails); low-risk network takeaways: multiple (attack) strategies exist, attackers deploy high-volume phishing servers in the cloud; High-risk network takeaways: Some bursty attacks come from smaller hosting providers (burstiness: implies anomoly detection could work), Some attackers use internet hosting providers and the same IP addresses over long periods of time (--> policy-based defenses, or this is the case were static blocklists are more effective).}


% This section discusses specific networks and IP addresses in both the low and high-risk category. % (as defined in \S\ref{sec:infrastructure}).
% First, we examine two prominent low-risk networks, 
% % namely the public cloud networks of Amazon~(\cref{sec:amazon}) and Microsoft~(\cref{sec:microsoft}).
% namely the public cloud networks of Amazon and Microsoft~(\S\ref{sec:case:low_risk}).
% Next, we explore two examples of high-risk networks, one that sends phishing emails in two bursts in a single month~(\S\ref{sec:case-study-bursty}) and one that remains high risk across the three months~(\S\ref{sec:case-study-persistent}). \todo{add 1 sentence motivating the case studies. perhaps also summarize the defensive takeaways given at each point, before the user gets bogged down in the details}

\subsection{Low-risk Networks}
\label{sec:case:low_risk}
\enew{We examine specific IP addresses in ranges owned by Amazon and Microsoft to better understand why ASes owned by these two large companies are the origins of a significant fraction (31\%) of all phishing email in our dataset (phishing still constitutes a low (<0.01\%) proportion of the total email these networks send, hence their low-risk classification as definined in \S\ref{sec:infrastructure}). Indeed, we find that attackers deploy high-volume phishing servers in the cloud and use multiple strategies when sending phish (such as account hijacking and email spoofing).}

% Move to the beginning of each AS subsection
%To better understand which cloud services are used for phishing, we matched the originating IP address of phishing emails to the published IP ranges for different cloud services of Amazon and Microsoft~\cite{AWSrange, Azurerange, Microsoft365range}. In Microsoft's case, we found a match for the IP addresses of 99.9\% of phishing emails. For Amazon, we were only able to determine what proportion of phishing emails came from AWS EC2 ranges (39.4\%), but were unable to identify other Amazon services for the remaining attacks.

% \enew{In \S\ref{sec:temporal}, we found that a large fraction of all phishing emails in our dataset originates from networks where phishing constitutes a low (<0.01\%) \textit{proportion} of the total email these networks send. Specifically two major hosting providers, Amazon and Microsoft, account for 31\% of the total phishing email traffic in January 2021. In the following case studies, we aim to shed light on potential explanations for the high amount of phishing emails originating from these major companies by examining specific IP addresses \footnote{Mapping IP addresses to cloud services: To better understand which cloud services are used for phishing, we matched the originating IP address of phishing emails to the published IP ranges for different cloud services of Amazon and Microsoft~\cite{AWSrange, Azurerange, Microsoft365range}. In Microsoft's case, we found a match for the IP addresses of 99.9\% of phishing emails. For Amazon, we were only able to determine what proportion of phishing emails came from AWS EC2 ranges (39.4\%), but were unable to identify other Amazon services for the remaining attacks.} within these companies.}

% old: 
% We classified a network as low risk if its outbound phishing probability is less than 10$\times$ that of the mean network’s probability (0.01\%). Despite sending mostly benign email, some of these networks are the source of a significant percentage of the phishing email in our dataset, with Amazon and Microsoft accounting for 31\%. 
% %---like Amazon and Microsoft, which combine to account for 31\% of the total phishing email traffic in Jan 2021. 
% Here, we discuss emails originating from Amazon and Microsoft in January 2021. %In these case studies we focused on examples of specific attack vectors, including a suspected dedicated phishing server, and a suspected compromised employee email account.

% I made this into a footnote as it's not very exciting and interrupts the flow of the section
% \paragraph{Mapping IP addresses to cloud services} 
% %Cloud providers host a variety of different services on their networks.
% To better understand which cloud services are used for phishing, we matched the originating IP address of phishing emails to the published IP ranges for different cloud services of Amazon and Microsoft~\cite{AWSrange, Azurerange, Microsoft365range}. 
% In Microsoft's case, we found a match for the IP addresses of 99.9\% of phishing emails.
% For Amazon, we were only able to determine what proportion of phishing emails came from AWS EC2 ranges (39.4\%), but were unable to identify other Amazon services for the remaining attacks.


\begin{figure*}[t]
    \centering
     \begin{subfigure}{0.35\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/comp-accnt-final.pdf}
        \subcaption{Suspected compromised email account from Amazon AS 16509.}
         \label{fig:accnt}
     \end{subfigure}\hspace{15ex}
     \begin{subfigure}{0.35\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/AWS-AC.pdf}
        \subcaption{Highest-volume phishing sender from Amazon AS 16509 and Microsoft AS 8075.}
         \label{fig:amazonAndMicrosoftSending}
     \end{subfigure}
     \begin{subfigure}{0.35\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/MIRHosting.pdf}
         \subcaption{Phishing emails from AS 52000.}
         \label{fig:burst}
     \end{subfigure}\hspace{15ex}
     \begin{subfigure}{0.35\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/9009Final.pdf}
         \subcaption{Phishing emails  from AS 9009.}
         \label{fig:m247}
     \end{subfigure}
     \vspace{-1em}
     \caption{Phishing over time for particular IP addresses and ASes during January 2021 (\S\ref{sec:caseStudies}).}
     \vspace{-1em}
\end{figure*}


\subsubsection{Amazon: AS 14618 \& AS 16509}\label{sec:amazon}
%The majority (60.63\%)  of phishing IP addresses from Amazon did not match specific cloud services.
%Of the ones that did match a listed service, 99.9\% corresponded to EC2. %, and these EC2 IP addresses sent 39.36\% of all phishing email from Amazon ASes in January 2021. 
% (7,623 out of a total of 26,983 phishing emails). 
%Both ASes saw about an equal amount of unmatched IP addresses, although we saw approximately double the number of phishing email originating from EC2's IP address ranges in AS 16509 (AS 16509: 5,288, AS 14618: 2,335 in January 2021). 
\enew{On aggregate, 39.36\% (7,623 emails) of all phishing email originating from Amazon's ASes come from a published EC2 IP address range (based on Amazon's published IP address ranges, we were unable to determine the other Amazon services for the remaining phishing emails)~\cite{AWSrange}.}
% \enew{Within Amazon's ASes, based on the aggregate email traffic from particular IP addresses, we observed two distinct phishing strategies: email account compromise and a ``phishing server" sending spoofed emails.}

%To better understand which cloud services are used for phishing, we matched the originating IP address of phishing emails to the published IP ranges for different cloud services of Amazon and Microsoft~\cite{AWSrange, Azurerange, Microsoft365range}. In Microsoft's case, we found a match for the IP addresses of 99.9\% of phishing emails. For Amazon, we were only able to determine what proportion of phishing emails came from AWS EC2 ranges (39.4\%), but were unable to identify other Amazon services for the remaining attacks.


\paragraph{Email account takeover}
\enew{In a potential instance of account hijacking, we found a significant volume of phishing email originating from a single Amazon IP address, where the \from address contained a legitimate corporate domain and a human-looking user name (\eg \textit{jane.smith$@$company.com}). The account sent 115 phishing emails to \cuda customers in January 2021, but did not send any phishing emails in January 2020 or October 2020. Moreover, this IP address sent 2,197 clean emails in January 2021, 1,460 clean emails in October 2020, and no emails in January 2020.}

% old
% Within Amazon's AS 16509, we observed that some phishing emails might have come from compromised accounts.
% In particular, in one potential instance of account hijacking, the \from address sent a significant volume of phishing emails from a legitimate corporate domain, and had a human-looking user name (\eg \textit{jane.smith$@$company.com}). 
% This email account was responsible for all phishing email from a single Amazon IP address. The account sent 115 phishing emails to \cuda customers in January 2021, but did not send any phishing emails in January 2020 or October 2020. Moreover, this IP address sent 2,197 clean emails in January 2021, 1,460 clean emails in October 2020, and no emails in January 2020.

%In addition, we did not see any other phishing emails from the same source IP address. 
%The IP ranges these phishing emails were sent from were not mapped to the AWS EC2 service.
%\grant{I'm not sure how this last sentence supports the compromised account conclusion, so I would either elaborate or remove it.}

Figure~\ref{fig:accnt} shows the number of phishing and clean emails customers received from this IP address throughout January 2021. Compared to other cases described below, this attack had a longer duration \enew{(of approximately 1 week)}, which matches the findings of prior work on compromised email accounts that shows that compromise incidents can last for days and even weeks~\cite{lateral1,lateral2}.


\paragraph{Dedicated phishing server sending spoofed emails} 
% todo: rewrite for clarity
\enew{The Amazon IP address responsible for sending the most phishing emails exhibited different behavior: In January 2021, customers received 1,324 phishing emails with 388 unique \from values where the address was \textit{noreply$@$domain.com} across multiple domains. As seen in the blue curve in Figure~\ref{fig:amazonAndMicrosoftSending}, all of the phishing emails from this IP address were sent within a short period of time. The IP address also sent 458 emails that \cuda did not classify as phishing and did not send phishing emails in the other time snapshots. The large burst of seemingly spoofed emails suggest the attackers either set up their own email server on AWS or compromised a legitimate server to send a large amount of phishing emails.}

% old
% The Amazon IP address responsible for sending the most phishing emails sent 1,324 phishing emails in January 2021 with 388 unique SMTP \from values where the address was \textit{noreply$@$domain.com} across multiple domains. The IP address also sent 458 emails that \cuda did not classify as phishing.
% This IP address did not send phishing emails in the other time snapshots. 
% %\grant{Because of the re-ordering, let's move the Microsoft noreply discussion here, and then move this sentence to the Microsoft section.}
% As seen in the blue curve in Figure~\ref{fig:amazonAndMicrosoftSending}, all of the phishing emails from this IP address were sent within a short period of time.
% The large burst of seemingly spoofed emails suggest the attackers either set up their own email server on AWS or compromised a legitimate server to send a large amount of phishing emails. 
%\grant{Hmmm, I'm not sure I follow why this last point results from the above analysis?}
% the phishing email sending pattern over time from this particular IP address. It also sent all its phishing emails within a short period of time. This pattern suggests that the attackers either set up their own email server on the Amazon cloud or compromised a legitimate server to send a larger number of attack emails. 

% note: compiled takeaways to the end of 5.2
% \paragraph{Takeaway: Multiple strategies exist} 
% The above case studies illustrate that attackers use different strategies, included compromising individual email accounts and compromising or standing up servers when sending spoofed emails. These strategies may benefit from individualized defenses. For example, compromised accounts may be detected by looking for unusual patterns in account activity~\cite{compAccoountsKdd2010}. 
% \vspace{-2ex}

% In our data, phishing emails sent via a compromised email account are much less common than campaigns that are sent from a dedicated phishing server that spoofs one or more email addresses. Since they are more common, we next consider in more detail another such dedicated server, this one hosted in Microsoft Azure.

%note from Elisa: We tried to determine the difference b/w account compromise and dedicated phishing server by number of unique from emails, but it didn't seem like there is a conclusive pattern as some attackers spoof many domains/emails while some only spoof 1. I think the paragraph above summarizes this. \ekb{It would be great to say how common each of these patterns is across the dataset. It seems like at least rough approximations of them could be checked programmatically. Can we at least check for ones based on phishing probability and variety of senders?}

\subsubsection{Microsoft: AS 8075}\label{sec:microsoft} 
Among the phishing emails from Microsoft's networks, we determined that 99.6\% came from Azure Cloud IP address ranges, with the rest from Exchange Online and Sharepoint. % not sure if this interrupts the flow / not sure why it is here when reading thru

\paragraph{Dedicated phishing server sending spoofed emails}  
% note: I rephrased this paragraph, still confusing though
\enew{Within AS 8075, we observe that the IP address that sent the most phishing emails behaves most like an attacker-controlled server. In total, this address (which falls within an Azure Cloud range) sent 2,465 phishing emails and 20 clean emails in January 2021, with 578 unique \from values, where the \from values for all the phishing emails are in the form of \textsc{noreply$@$domain} with different domains. 
Given the high number of emails, the wide-range of unique domains, and the generic \textsc{noreply$@$} addresses, this scenario is most consistent with an attacker using email spoofing to forge sender names. Furthermore, as seen in the orange curve in Figure~\ref{fig:amazonAndMicrosoftSending}, this IP address exhibited a ``bursty'' email sending behavior, similar to the second Amazon case study (the blue curve), and we did not find any phishing email from this IP address in the 2020 datasets.}

% old
% Within AS 8075, we examined the IP address that sends the most phishing. The IP address is mapped to Azure Cloud. We found a total of 2,465 phishing emails and 20 clean emails sent from this address in January 2021, with 578 unique SMTP \from values. 
% The \from values for all the phishing emails are in the form of \textsc{noreply$@$domain} with different domains. 
% %\grant{Can we give a ballpark number and replace the ``many different'' with ``N different''?} 
% Given the high number of emails, the wide-range of unique domains, and the generic \textsc{noreply$@$} addresses, 
% this scenario is most consistent with an attacker using email spoofing to forge sender names.
% %we concluded that this attacker was likely using email spoofing to forge the sender name. 
% As seen in the orange curve in Figure~\ref{fig:amazonAndMicrosoftSending}, this IP address exhibited a ``bursty'' email sending behavior, similar to the second Amazon case study (the blue curve). 
% %That is, all the phishing emails from this IP address were sent in the span of a few hours.
% We did not find any phishing email from this IP address in the 2020 datasets.

%We know that this attacker sent a high volume of phishing email within a short amount of time using a server hosted on Microsoft Azure Cloud, and likely used spoofing to impersonate all kinds of trustworthy/legitimate domains (.edu domains, for example). 


% compiling the takeaways for low-risk networks / reiterating motivations
% (added takeaway from 5.1.1)
\paragraph{Takeaway 1: Multiple strategies exist} 
The above case studies illustrate that attackers use different strategies, including compromising individual email accounts and compromising or standing-up servers to send spoofed emails. These strategies may benefit from individualized defenses. For example, compromised accounts may be detected by looking for unusual patterns in account activity~\cite{compAccoountsKdd2010}. 

\paragraph{Takeaway 2: Attackers deploy high volume phishing servers in the cloud} %, but common attack patterns may be a basis for defenses} 
\label{sec:defense-from-bursts}
The fact that the highest volume servers send their attacks in such short bursts~(Figure~\ref{fig:amazonAndMicrosoftSending}) suggests that they may be shut down after a short time \textit{and} that the pattern may be exploited as part of detection. Cloud providers  could use these patterns as a signal to identify VMs potentially abused for sending malicious email. Similarly, enterprise email defenses can potentially quarantine large email bursts from a previously-unseen sending server. \enew{This attack strategy also illustrates the limitations of using purely network-reputation-based defenses against phishing.}


\subsection{High-risk Networks}
\label{sec:caseStudy_highRisk}
\enew{In \S\ref{sec:temporal} we find that while attackers consistently reuse some networks to send phishing emails, some phishing email delivery infrastructure is short-lived. Here, we propose explanations and possible defenses for the different network behaviors we observe by investigating} two high-risk networks: one that sends phishing emails during only one month in our dataset (and displayed similar patterns to our Amazon and Microsoft case studies), and one that consistently sends many phishing emails over the three time periods.


\begin{table}[t]
\centering
\footnotesize
\begin{tabular}{|l|l|l|}
\hline
\textbf{Time Period} & \textbf{\# Phishing} & \textbf{\# Clean} \\ \hline
Jan 2020 & 955  & 29099 \\ \hline
Oct 2020 & 3207 & 47560 \\ \hline
Jan 2021 & 2135 & 8685  \\ \hline
\end{tabular}
\caption{Clean and phishing email volume over time of AS 9009.}
     \vspace{-2em}
\label{tab:persistent-case-study}
\end{table}

% \begin{figure}[t]
%     \centering
%     \includegraphics[width=0.8\columnwidth]{figures/m247dist.pdf}
%     \caption{Cumulative fraction of phishing email over IP addresses within AS 9009, ranked by phishing email volume.
%     \grant{TODO: I think we can cut this graph. I think the only place we reference it is in 5.2.2, which says that the top 32 IP addresses each send 20+ emails. For space reasons, we can just say that and omit the graph.}
%     }
%     \label{fig:m247dist}
% \end{figure}

\begin{table}[t]
\centering
\footnotesize
\begin{tabular}{|l|l|l|}
\hline
\textbf{Phishing Lifespan} &
  \textbf{\# Phishing} &
  \textbf{\# Clean} \\ \hline
15 days 11:59:34 & 245 & 10 \\ \hline
1 days 16:32:37  & 127 & 19 \\ \hline
0 days 09:10:08  & 96  & 2  \\ \hline
10 days 12:38:23 & 81  & 0  \\ \hline
9 days 08:24:46  & 71  & 2  \\ \hline
1 days 17:15:40  & 71  & 0  \\ \hline
7 days 23:46:46  & 67  & 88 \\ \hline
21 days 03:07:51 & 64  & 4  \\ \hline
0 days 05:47:59  & 60  & 3  \\ \hline
0 days 01:03:14  & 53  & 0  \\ \hline
\end{tabular}
\caption{Phishing sending lifespan and email volume for the top-10 phishing senders by IP within AS 9009 in January 2021.}
\label{fig:top10-9009}
\vspace{-5ex}
\end{table}

\subsubsection{Bursty High-risk Network: AS 52000}
\label{sec:case-study-bursty}
We saw two large bursts in January 2021 (Figure~\ref{fig:burst}) comprising a total of 1,673 phishing emails from AS 52000, a Russian hosting company with data centers in the Netherlands, Russia, and the U.S.; no other emails in our dataset originate from this network during that month.
The phishing emails come from 20 unique IP addresses and span 533 campaigns (as defined by same subject and \from).
Attackers used the phishing IP addresses from AS 52000 for very short lifetimes:
% The phishing IP addresses from AS 52000 are all extremely short-lived: 
across the entire month, these addresses actively send phishing emails for less than 24 hours total; and the highest volume senders among these IP addresses send all of their phishing emails within short 30 minute windows.
% - all sending their phishing emails within the span of less than 24 hours - for an average phishing email lifespan of 12.5 hours.
% Similarly, the top senders by IP address have a lifespan as short as 30 minutes. %\elisa{I think it's hard to tell if the two bursts are actually different attackers based on the information we have}.
No phishing emails originated from this AS outside of these two bursts in Jan 2021.
% Outside of these two these bursts, this AS did not send any phishing emails in the other time periods.
This behavior suggests an attacker who abuses cloud hosted servers to send large bursts of phishing emails, before switching to new infrastructure (\eg because a provider terminates their services).
% In this network, the attackers are likely sending a large burst of phishing email (with many different campaigns) before getting shut down.
% TODO: change writing?


% moving takeaways to be compiled at the end
% \paragraph{Takeaway: Some bursty attacks come from smaller hosting providers (not just the cloud providers)}
% A time-series-based anomaly detector that analyzes the volume of a particular network's email traffic could potentially flag periods of higher phishing risk.
% Smaller hosting companies could benefit from such tools to flag suspect servers.

% \vspace{-2ex}
\subsubsection{Persistent High-risk Network: AS 9009}\label{sec:case-study-persistent}
Our final case study examines AS 9009, which belongs to a UK-based hosting company. \enew{We observed a consistently high volume and proportion of phishing email originating from this network; as shown in Table~\ref{tab:persistent-case-study}, AS 9009 was one of the 9 networks we classified as high-risk for all three time periods. 
In contrast to the bursty behavior observed in the prior case studies, we find (Figure~\ref{fig:m247}) that phishing attacks regularly originated from this network throughout the month of January 2021 (the other months in our data had similar distributions). 
The phishing emails from AS 9009 span 1,031 unique phishing campaigns and come from 151 unique IP addresses, where 32 of these IP addresses send over 20 phishing emails each. 
One reason for the high number of unique phishing IP addresses and campaigns might be that multiple attackers use this AS to send phishing emails.}

To shed light on the volatility of the phishing IP addresses within AS 9009, we calculated the phishing email sending lifespan of each IP address, \ie the time between the first phishing email we saw from the IP address to the last phishing email (because we compute this duration over 1 month windows, the maximum lifespan is 31 days). In January 2021, the average lifespan of a phishing IP address from this AS is 41.5 hours. However, as shown in Table~\ref{fig:top10-9009}, many of the IP addresses with the highest phishing volumes continuously send phishing emails for extended periods of time. Given that relatively low volumes of clean email originate from each of these same high phishing volume IP addresses, they likely correspond to dedicated phishing servers.

% old: 
% In addition, we find (Figure~\ref{fig:m247}) that attackers regularly sent phishing emails from this network throughout January 2021 (the other months in our data had similar distributions), different from the bursty behavior observed in the prior case studies. In January 2021, the phishing emails from AS 9009 span 1,031 unique phishing campaigns and come from 151 unique IP addresses, where 32 of these IP addresses send over 20 phishing emails each. One reason for the high number of unique phishing IP addresses and campaigns might be that multiple attackers use this AS to send phishing emails.

% old: As summarized in Table~\ref{tab:persistent-case-study}, this AS consistently had a high phishing probability and sent a large volume of phishing in all three time periods, leading to a high-risk classification in each month.
% In addition, we find (Figure~\ref{fig:m247}) that attackers regularly sent phishing emails from this network throughout January 2021 (the other months in our data had similar distributions), different from the bursty behavior observed in the prior case studies.

% old and old comments
% The number of phishing emails over time sent by this AS is depicted in Figure~\ref{fig:m247}, while Table~\ref{tab:persistent-case-study} shows the clean and phishing email volume over time. The results shows that this AS consistently has an elevated probability of phishing, leading it to be classified as high risk in all 3 time periods. 
% \Cref{fig:m247} shows that this AS was the source of phishing email regularly throughout January 2021 (and had a similar distribution across the other months), as opposed to sending in large, short-lived bursts like the prior ASes we examined.
% sending in large, short-lived bursts in the previous examples from Microsoft~(\cref{fig:microsoftsending}) and Amazon~(\cref{fig:amazonsending}). 
% In January 2021, the phishing emails from AS 9009 span 1,031 unique phishing campaigns and come from 151 unique IP addresses, where 32 of these IP addresses send over 20 phishing emails each. 
% Figure~\ref{fig:m247dist} shows the distribution of phishing email by sender IP address within this AS. There are 32 unique sender IP addresses that each had more than 20 phishing emails originating from them. 
% One reason for the high number of unique phishing IP addresses and campaigns might be that multiple attackers use this AS to send phishing emails.

% The high number of unique phishing IP addresses and campaigns suggests that there are likely to be multiple attackers using servers within this AS to send phishing email. 

% old 
% To shed light on the volatility of the phishing IP addresses within AS 9009, we calculated the phishing email sending lifespan of each IP address, \ie the time between the first phishing email we saw from the IP address to the last phishing email (because we compute this duration over 1 month windows, the maximum lifespan is 31 days).
% In January 2021, the average lifespan of a phishing IP address from this AS is 41.5 hours.
% However, as shown in Table~\ref{fig:top10-9009}, many of the IP addresses with the highest phishing volumes continuously send phishing emails for extended periods of time.
% % Although some of the highest-volume phishing email senders within AS 9009 are still short-lived, many of them send phishing email continuously for an extended period of time. 
% Given that relatively low volumes of clean email originate from each of these same high phishing volume IP addresses, they likely correspond to dedicated phishing servers.

% compiling takeaways at the end
\paragraph{Takeaway 1: Some bursty attacks come from smaller hosting providers (not just the cloud providers)}
A time-series-based anomaly detector that analyzes the volume of a particular network's email traffic could potentially flag periods of higher phishing risk.
Smaller hosting companies could benefit from such tools to flag suspect servers.

\paragraph{Takeaway 2: Some attackers use Internet hosting providers and the same IP addresses over long periods of time} %, via the same IP addresses}
This long-lived malicious behavior suggests the need to adopt additional technical or policy-based defenses to help curtail attacks coming from such networks.

% \todo{Make takeaways crisper and add conclusion + segway into section 6}
% i.e., what do we want readers to get out of this section? what do we really shed light on here? it doesn't have to be revolutioary, just make it clear if the reader had to takeaway one thing, then what
